Kaon decays and other hadronic processes in lattice QCD

This thesis deals with the study of properties and interactions of light mesons. Specifically, we focus on hadronic decay and scattering processes, which are dominated by effects of the strong interaction in the low-energy regime. A peculiarity of the strong interaction is that perturbative expansions fail at hadronic energy scales. Thus, genuine nonperturbative tools are essential to obtain first-principles predictions. Here we use Lattice Field Theory, and Effective Field Theories. The mathematical formulation of Quantum Chromodynamics (QCD) and the methods to resolve its dynamics will be addressed in Chapter 1. The research of this dissertation is divided in two parts. Chapter 2 describes our study of the 't Hooft limit of QCD using lattice simulations, while in Chapter 3 we consider processes that involve multiparticle states. The 't Hooft limit provides a simplification of nonabelian gauge theories that leads to nonperturbative predictions. We will analyze the scaling with the number of colours of various observables, such as meson masses, decay constants and weak matrix elements. A question we address is the origin of the long-standing puzzle of the $\Delta I=1/2$ rule, that is, the large hierarchy in the isospin amplitudes of the $K \to \pi\pi$ weak decay. Regarding multiparticle processes, we will discuss generalizations of the L\"uscher formalism to explore three-particle processes from lattice simulations. The focus will be on our contributions, such as our implementation of the finite-volume formalism that includes higher partial waves, and the first application of the formalism to a full lattice QCD spectrum. We will also comment on the extension of the approach to generic three-pion systems. A summary in Spanish will be given in Chapter 4. The final part of the thesis (Part II) includes the peer-reviewed publications in their original published form.

==> Chapters/Resumen_Tesis/Resumen_Tesis.tex <==

\chapter{Resumen de la tesis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




